Geometric Fault-Tolerant Control of Quadrotors in Case of Rotor Failures: An Attitude Based Comparative Study

The ability of aerial robots to operate in the presence of failures is crucial in various applications that demand continuous operations, such as surveillance, monitoring, and inspection. In this paper, we propose a fault-tolerant control strategy for quadrotors that can adapt to single and dual complete rotor failures. Our approach augments a classic geometric tracking controller on $SO(3)\times\mathbb{R}^3$ to accommodate the effects of rotor failures. We provide an in-depth analysis of several attitude error metrics to identify the most appropriate design choice for fault-tolerant control strategies. To assess the effectiveness of these metrics, we evaluate trajectory tracking accuracies. Simulation results demonstrate the performance of the proposed approach.

==> symbol_list.tex <==
%!TEX root = ARTICLE.tex
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}
\DeclareMathOperator{\Diag}{Diag} 
%%%%%%%%%%%%% Comando para glosario %%%%%%%%%%%%%%55
\newcommand{\glo}[3]{
%#1: id
%#2: name
%#3: 
	\newglossaryentry{#1}
	{
	  name=#2,
	  description=#3,
	}
}
%%%%%%%%%%%%%%% Comando para definir un simbolo%%%%
\newcommand{\glom}[4]{
%#1: id
%#2: name
%#2: Symbol
%#3: description
	\newglossaryentry{#1}
	{
	  name={\ensuremath{#2}},
	  symbol={\ensuremath{#3}},
	  description=#4,
	  type=symbols,
	}
}
%%%%%%%%%%%%%%% Comando para definir un simbolo%%%%
\newcommand{\glomh}[4]{
%#1: id
%#2: name
%#2: Symbol
%#3: description
	\newglossaryentry{#1}
	{
	  name={\ensuremath{#2}},
	  symbol={\ensuremath{#3}},
	  description=#4,
	  %type=hidden,
	}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\glo{naiive}{naive}{ratio of circumference of circle to its
               diameter}



%%http://tex.stackexchange.com/questions/236670/custom-glossary-style-makenoidxglossaries-and-glsgroupskip


%% Linear model
\glomh{linx}{A}{A}{Input matrix.}
\glomh{linp}{C}{C}{parameter matrix.}


% dynamics
\glom{sgn}{\chi}{\chi}{Indicator function}
\glom{error}{e}{e}{Desired roll}
% \glom{droll}{\phi^*}{\phi^*}{Desired roll}
\glom{roll}{\phi}{\phi}{roll}
\glom{pitch}{\theta}{\theta}{pitch}
\glom{yaw}{\psi}{\psi}{yaw}
\glom{droll}{ p}{ p}{roll}
\glom{dpitch}{ q}{ q}{pitch}
\glom{dyaw}{ r}{ r}{yaw}
\glom{angles}{\mathbf{\Theta}}{\mathbf{\Theta}}{Robot attitude}
\glom{dangles}{\mathbf{\Omega}}{\mathbf{\Omega}}{Angular velocities}
\glom{id}{k}{k}{general id of robot used in description of control method and estimation}

\glom{thrust}{F}{F}{Thrust}
\glom{u}{\mathbf{u}}{\mathbf{u}}{control input}
\glom{w}{\mathbf{w}}{\mathbf{w}}{control input}
\glom{angular}{\omega}{\omega}{angular speed}

% Coordinate frames
\glom{worldf}{\mathcal{I}}{\mathcal{I}}{World frame}
\glom{loadf}{\mathcal{L}}{\mathcal{L}}{Load frame}
\glom{robotf}{\mathcal{B}}{\mathcal{B}}{Body frame}
\glom{camf}{\mathcal{C}}{\mathcal{C}}{Camera frame}

%\glom{tagf}{\mathpzc{T}}{\mathpzc{T}}{Tag frame}
%\glom{dockf}{\mathpzc{d}}{\mathpzc{d}}{Docking module frame}
%\glom{camf}{\mathpzc{C}}{\mathpzc{C}}{Camera frame}
%\glom{waitf}{\mathpzc{w}}{\mathpzc{w}}{Waiting module frame}

%% Robots
\glom{tag}{\mathpzc{t}_p}{\mathpzc{t}_p}{Tag}
\glom{robots}{\mathcal{R}}{\mathcal{R}}{Set of a team of robots}
\glom{robotl}{\mathbf{x}}{\mathbf{x}}{Robot location.}
\glom{robot}{\mathbf{x}}{\mathbf{x}}{Robot location.}
\glom{width}{\mathpzc{w}}{\mathpzc{w}}{Robot width.}
\glom{height}{\mathpzc{h}}{\mathpzc{h}}{Robot height.}
\glom{orientations}{\Psi}{\Psi}{Robot orientations.}
\glom{orientation}{\psi}{\psi}{Robot orientation.}
\glom{structure}{\mathit{S}}{\mathit{S}}{Structure}
\glom{structureset}{\mathcal{S_F}}{\mathcal{S_F}}{Structure set}
\glom{component}{\mathit{S}}{\mathit{S}}{Structure}

% Desired structure
\glom{targets}{\mathcal{Z}}{\mathcal{Z}}{Target points}
\glom{targetse}{\mathcal{Z}^E}{\mathcal{Z}^E}{Expanded target points}
\glom{target}{z}{z}{Robot location.}

\glom{tree}{\mathcal{T}}{\mathcal{T}}{Assembly tree.}
\glom{tedges}{\mathcal{E}^\mathcal{T}}{\mathcal{E}^\mathcal{T}}{Edges of the Assembly tree.}
\glom{tvertices}{\mathcal{V}^\mathcal{T}}{\mathcal{V}^\mathcal{T}}{Vertices of the Assembly tree.}
\glom{tivertices}{\mathcal{V}^{\mathcal{T}_i}}{\mathcal{V}^{\mathcal{T}_i}}{Vertices of the Assembly tree.}

\glom{graph}{\mathcal{G}}{\mathcal{G}}{Communication graph}
\glom{cgraph}{\hat{\mathcal{G}}}{\hat{\mathcal{G}}}{Canonical robust graph}
\glom{vertices}{\mathcal{V}}{\mathcal{V}}{Set of Vertices}
\glom{neighbors}{\mathcal{N}_i}{\mathcal{N}}{Neighbors for node $i$}
\glom{edges}{\mathcal{E}}{\mathcal{E}}{Set of Edges}
\glom{neighborsi}{\mathcal{J}_i}{\mathcal{J}}{Inclusive Neighbors for node $i$}
\glom{removed}{\mathcal{R}}{\mathcal{R}}{Removed nodes}
\glom{normal}{\mathcal{N}}{\mathcal{N}}{Normal nodes}
\glom{strongset}{\mathcal{F}}{\mathcal{F}}{Strong nodes}
\glom{weakset}{\mathcal{W}}{\mathcal{W}}{Weak nodes}
\glom{candidates}{\mathcal{C}}{\mathcal{C}}{Candidate points}
\glom{boundary}{\mathcal{P}}{\mathcal{P}}{Objective points}

\glom{loc}{v}{v}{Node location in the space}
\glom{val}{x}{x}{Variable of interest of the node}

\glom{received}{\mathcal{P}_i^t}{\mathcal{P}}{Set of received values by node $i$ a the time interval 
%$[t-T\, t]$
}


